Machine learning-guided directed evolution for protein engineering

Machine learning (ML)-guided directed evolution is a new paradigm for biological design that enables optimization of complex functions. ML methods use data to predict how sequence maps to function without requiring a detailed model of the underlying physics or biological pathways. To demonstrate ML-guided directed evolution, we introduce the steps required to build ML sequence-function models and use them to guide engineering, making recommendations at each stage. This review covers basic concepts relevant to using ML for protein engineering as well as the current literature and applications of this new engineering paradigm. ML methods accelerate directed evolution by learning from information contained in all measured variants and using that information to select sequences that are likely to be improved. We then provide two case studies that demonstrate the ML-guided directed evolution process. We also look to future opportunities where ML will enable discovery of new protein functions and uncover the relationship between protein sequence and function.

==> comparison_table.tex <==
\begin{table}
\caption{Selected studies using machine learning to guide directed evolution}
	\begin{tabular}{r r r r r}
		\hline
\textbf{Protein} & \textbf{Property} & \textbf{\textit{n} screened} & \textbf{Model}\\
		\hline 
		halohydrin dehydrogenase & volumetric productivity & 60,000 & linear\cite{fox2003optimizing_note,fox2005directed,fox2007improving}
\\
        epoxide hydrolase & enantioselectivity & 20,000 & ASRA\cite{feng2012enhancing}\\
        proteinase K & activity, heat tolerance & 95 & linear\cite{liao2007engineering}\\
        glutathione transferase  & catalytic activity & 95 & linear\cite{govindarajan2014mapping}\\
   		glutathione transferase  & catalytic activity & 95 & linear\cite{musdal2017exploring}\\
        cytochrome P450 & thermostability & {\raise.17ex\hbox{$\scriptstyle\sim$}}200 & GP\cite{romero2013navigating_note}\\
        channelrhodopsin & membrane localization & {\raise.17ex\hbox{$\scriptstyle\sim$}}200 & GP\cite{bedbrook2017machine}\\
        green fluorescent protein & fluorescence & 296 & GP\cite{saito2018machine}\\
        channelrhodopsin & spectral properties & 119 & GP\cite{bedbrook2017minimally}\\
		\hline
	\end{tabular}\\
    \label{tab:ml}
\end{table}
